Towards Full Automated Drive in Urban Environments: A Demonstration in GoMentum Station, California

Each year, millions of motor vehicle traffic accidents all over the world cause a large number of fatalities, injuries and significant material loss. Automated Driving (AD) has potential to drastically reduce such accidents. In this work, we focus on the technical challenges that arise from AD in urban environments. We present the overall architecture of an AD system and describe in detail the perception and planning modules. The AD system, built on a modified Acura RLX, was demonstrated in a course in GoMentum Station in California. We demonstrated autonomous handling of 4 scenarios: traffic lights, cross-traffic at intersections, construction zones and pedestrians. The AD vehicle displayed safe behavior and performed consistently in repeated demonstrations with slight variations in conditions. Overall, we completed 44 runs, encompassing 110km of automated driving with only 3 cases where the driver intervened the control of the vehicle, mostly due to error in GPS positioning. Our demonstration showed that robust and consistent behavior in urban scenarios is possible, yet more investigation is necessary for full scale roll-out on public roads.

==> ack.tex <==
\vspace{-0.25cm}

\section{\footnotesize{Acknowledgments}}

\footnotesize{Authors would like to thank Paul Cummings, Kikuo Fujimura and Sue Bai of Honda for their support and making this demonstration possible.}

\vspace{-0.1cm}

==> jhuang.tex <==
\section{Perception}

TODO: Akansel
 
Length: 0.25 column

\subsection{Localization}

TODO: Alex

Length: 0.5 column

\subsection{Pedestrian Detection \& Tracking}

TODO: Jiawei

Length: 0.5 column

The goal of the pedestrian detector is to accurately detect pedestrians' position and velocity in 3D. It consists of three stages. The first stage is pure vision-based pedestrian detection. We first extract HOG features from the image at different scales. The extracted features are then classified by a linear SVM followed by an RBF. Adding the RBF is crucial because it significantly increases the discriminatory power of the classifier. Both classifiers are trained on 5000 positive samples and iteratively trained with hard negative samples. The ouput of this stage is a set of bounding boxes and corresponding scores indicating the probability of containing a pedestrian. To reduce false-positive rate, we discard any bounding box which scores below an empirically derived threshold of 0.5.

The second stage is lidar association. Since the relative pose between lidar and camera has been calibrated, we project all the lidar points located in front of the camera onto the image. Then for each pedestrian bounding box detected in the first stage, we find all the lidar points inside the bounding box area. Among these points, we pick the one closest to our ego vehicle and assign the coordinates of that point to the bounding box. The reason is that only the closest lidar point actually belongs to the pedestrian. Points that are more distant belong to the background behind the pedestrian. The point also cannot belong to a closer non-pedestrian object, otherwise that object will occlude the pedestrian and the bounding box would not be detected in the first stage. After each bounding box's relative coordinates are assigned, we perform several filtering steps -- bounding boxes which fail any all of the criteria will be eliminated: the box must not be entirely be above the horizon line, the box must have typical aspect ratio of a person, the box must have normal sizes at the given distance and the box must have at least one lidar point inside. The remaining bounding boxes are passed to the third stage. After this step, a pedestrian will be treated as a point.

The third and last stage is the linear tracker. Tracking serves two purposes: 1) it generates an estimate of pedestrian velocity; 2) it performs non-maximum suppression since multiple bounding boxes can result from a single pedestrian in the previous step. Tracking should be performed in a fixed world frame, thus we must transform all the vehicle-relative coordinates into a global frame. After the transformation, we use a linear motion model to track the pedestrian. The algorithm works as follows: first we cluster all the points. If a cluster is close enough to an existing tracker's latest position, it is considered the latest observation for that tracker and be added to that tracker. The tracker's trajectory equation is then updated to the least-square fit linear curve of all the assigned observations. If a cluster does not lie close to any existing tracker, we create a new tracker for it. In addition, we delete any tracker that has not received any update in a given timeframe because we believe the object has disappeared or lost track.

The final output of the pedestrian detection module is the current position and velocity of all tracked pedestrians. These are eventually consumed by the event handler to raise a pedestrian event.

\subsection{Vehicle Detection \& Tracking}

TODO: Jiawei, Lichao

Length: 1 column

One challenging but important task for any autonomous vehicle at an intersection is to detect cross traffic from distance. In our demo we want to detect cross traffic vehicle 150m away. At this distance, camera is not effective because the target car appears too small in the image. Even lidar cannot reach that distance. Here we present a radar-based cross traffic detection technique.

We used Delphi ESR radar which combines two operating modes: long-range narrow-angle mode and mid-range wide-angle mode. The device alternates between the two modes at a frequency of 40Hz. By assemblying the two consecutive scans, we create a full scan at a frequency of 20Hz. In the long-range mode, the radar can detect up to 175m which is ideal for our long range requirement.

The radar points are first filtered by their velocity, x/y position and signal strength. The filtered points are then clustered. Depending on their position, each cluster either gets assigned to an existing tracker or generates a new tracker. We use particle filter as our backend tracking algorithm. Particle filter requires a state model and a measurement model. We adopted the formulations in \ref{}.

Each tracked vehicle is represented by a state vector $x_k = [x, y, v, heading, raw\ rate]$. For our vehicle to respond to the crossing vehicle, we have to convert the state vector into an actionable metric. We chose time-to-collision (TTC) as such a metric. TTC is defined as the time before the crossing vehicle passes our ego vehicle. To compute the TTC, we first compute the closing velocity of the crossing traffic (e.g. when the cross traffic is left-right direction, the closing velocity is the vehicle's velocity component in the left-right direction). Then the TTC is calculated as $d_{closing} / v_{closing}$, where $d_{closing}$ is the lateral distance in the left-right direction. Due to the noisy nature of the tracker output, TTC computed above is not always monotonically decreasing. Therefore, we added an "extrapolation" logic in our TTC calculation -- for a short duration, if the TTC calculated from tracker output is higher than last published TTC, we will instead use TTC extrapolated from previous TTC values. The goal of this step is to provide some noise tolerance to sporadic erroneous tracker output. The final published TTC will be used by the event handler to determine the vehicle GO/STOP action.

[A Direct Scattering Model for Tracking Vehicles with High-Resolution Radars, Christina Knill]


\subsection{Obstacle Detection \& Tracking}

TODO: Mahmut

Laser-based detection

Length: 0.5 column

\subsection{DSRC-based Detection}

TODO: Hasan

Two use cases: V2V and V2P

Length: 0.25 column


